Self-Sampling for Neural Point Cloud Consolidation

We introduce a novel technique for neural point cloud consolidation which learns from only the input point cloud. Unlike other point upsampling methods which analyze shapes via local patches, in this work, we learn from global subsets. We repeatedly self-sample the input point cloud with global subsets that are used to train a deep neural network. Specifically, we define source and target subsets according to the desired consolidation criteria (e.g., generating sharp points or points in sparse regions). The network learns a mapping from source to target subsets, and implicitly learns to consolidate the point cloud. During inference, the network is fed with random subsets of points from the input, which it displaces to synthesize a consolidated point set. We leverage the inductive bias of neural networks to eliminate noise and outliers, a notoriously difficult problem in point cloud consolidation. The shared weights of the network are optimized over the entire shape, learning non-local statistics and exploiting the recurrence of local-scale geometries. Specifically, the network encodes the distribution of the underlying shape surface within a fixed set of local kernels, which results in the best explanation of the underlying shape surface. We demonstrate the ability to consolidate point sets from a variety of shapes, while eliminating outliers and noise.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-sigconf-authordraft.tex \
	samples/sample-sigconf-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-sigconf-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done

samples/sample-manuscript.pdf \
samples/sample-acmsmall.pdf \
samples/sample-acmlarge.pdf \
samples/sample-acmtog.pdf: samples/samplebody-journals.tex

samples/sample-sigconf.pdf \
samples/sample-sigconf-authordraft.pdf \
samples/sample-sigconf-xelatex.pdf \
samples/sample-sigplan.pdf \
samples/sample-sigchi.pdf: samples/samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean
	$(RM) $(PDF) samples/*-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> ablation.tex <==
\section{Ablations}


\subsection{Beam-Gap Loss}
To illustrate the effect of the beam-gap loss, we show a qualitative comparison with and without beam-gap in Figure~\ref{fig:beamgap}. This shows that convergence is quicker and better using the beam-gap loss.
\input{figures/07_ablation/beam_gap}

\subsection{Fixed Random Input}
The network receives a fixed random vector $C_l$ as input. This promotes the natural discriminative power of neural networks, which we want to leverage as a self-prior. To highlight this, we reconstruct a mesh using a fixed random vector $C_l \sim \mathcal{U}[0,1)$, and as a fixed constant vector $C_l = 0.1$ in Figure~\ref{fig:randomc}. Note that the results displayed are from iteration 4100 \revb{(converged result in main paper Figure 8)}, and the reconstruction from fixed constant vector will eventually improve in later iterations (\emph{e.g.,} enter between the legs of the cat). However, the result using fixed-random is (marginally) better. \revb{Due to the similarity in the final results of different setups, we display the intermediate results to highlight differences in convergence.}
\input{figures/07_ablation/random_vec}

\subsection{Increasing Sampling Resolution}
The amount of points sampled from the reconstructed mesh affects the speed of convergence. Sampling many points will increase convergence rapidly, which may make the optimization more susceptible to local minima. See an example in Figure~\ref{fig:sampling}. While all three configurations converge to a good result eventually, the configuration which ranges from 40k-70k points is (marginally) the best. \revb{Note that the sampling range of 70k means there was no increasing sampling resolution. The final converged result can be seen in the main paper (Figure 6).}
\input{figures/07_ablation/sampling}

==> figures/001_intro/teaser/lamp-ear.tex <==
\begin{figure}[h]
    \centering
    \newcommand{\pl}{-1}
    \begin{overpic}[width=0.75\columnwidth]{figures/001_intro/teaser/lamp-ear.jpg}
    \put(20,  \pl){\textcolor{black}{EAR}}
    \put(60, \pl){\textcolor{black}{ours}}
    \end{overpic}
    \caption{Comparison to EAR~\shortcite{huang2013edge}.}
    \label{fig:earcomp}
\end{figure}

==> figures/004_experiments/aliens/alien-points.tex <==
\begin{figure}
    \centering
    
    \includegraphics[width=\columnwidth]{figures/004_experiments/aliens/alien-points.jpg}
    
    \caption{Noisy input from the COSEG dataset . In orange is a \textit{single output} of our network emphasising edges, on the right is a dense $\times 10$ up-sampling obtained through multiple outputs.  }
    \label{fig:alien_points}
\end{figure}

==> figures/004_experiments/aliens/alien2.tex <==
\begin{figure}
    \centering
    
    \includegraphics[width=\columnwidth]{figures/004_experiments/aliens/alien2.jpg}
    
    \caption{Noisy input from the COSEG dataset . In orange is a non-dense output of our network showing emphasis on edges, on the right is a dense $\times 10$ up-sampling obtained through multiple outputs. }
    \label{fig:alien2}
\end{figure}

==> figures/004_experiments/density/limbs/leg-mesh.tex <==

\begin{figure}
    \centering
    \newcommand{\pl}{-4}
    \includegraphics[width=\columnwidth]{figures/004_experiments/density/limbs/leg-mesh.png}
    \begin{overpic}[width=\columnwidth, trim=0 0 0 0 ]{figures/004_experiments/density/limbs/hand-mesh.png}
    \put(20,  \pl){\textcolor{black}{Input}}
    \put(70, \pl){\textcolor{black}{Consolidated}}
    \end{overpic}
    \caption{\gm{Mesh Reconstruction of the real scanned hand (top) foot (bottom). }}
    \label{fig:leg_mesh}
\end{figure}

==> figures/004_experiments/density/synt/mesh/tiki.tex <==
\begin{figure}
    \centering
    \newcommand{\pl}{-4}
    \includegraphics[width=\columnwidth]{figures/004_experiments/density/synt/mesh/netta.png}
    \includegraphics[width=\columnwidth]{figures/004_experiments/density/synt/mesh/candle.png}
    \begin{overpic}[width=\columnwidth, trim=0 0 0 0 ]{figures/004_experiments/density/synt/mesh/tiki.png}
    \end{overpic}
    \caption{\gm{Consolidation of non-uniform sampled point clouds from meshes. Observe how in the first example, there is an entire patch that does not contain a single point. Because our method learn from present points it is not able to complete this patch.}}
    \label{fig:extra_mesh_density}
\end{figure}

==> figures/004_experiments/knife.tex <==
\begin{figure}[b]
    \centering
    \newcommand{\pl}{-2}
    \begin{overpic}[width=\columnwidth]{figures/004_experiments/knife.jpg}
    \put(12,  \pl){\textcolor{black}{Input}}
    \put(44, \pl){\textcolor{black}{EC-Net}}
    \put(78, \pl){\textcolor{black}{\ourmethod{}}}
    \end{overpic}
    \caption{Using simulated scanned point cloud as input (from~\cite{yu2018ec}), results of \ourmethod{} and the edge selected output from EC-Net. Results are directly output from the networks (without any pre/post processing).}
    \label{fig:knife_comparison}
\end{figure}

==> figures/004_experiments/sparse/bunny.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{figures/004_experiments/sparse/bunny.jpg} 
    \caption{Stanford bunny with 50K points as input up-sampled to 600K points.}
    \label{fig:bunny}
\end{figure}

==> figures/004_experiments/sparse/plane.tex <==
\begin{figure}[H]
    \centering
    \newcommand{\pl}{-2}
    \begin{overpic}[width=\columnwidth]{figures/004_experiments/sparse/plane.jpg}
    \put(12,  \pl){\textcolor{black}{Input}}
    \put(48, \pl){\textcolor{black}{$p_T=0.6$}}
    \put(78, \pl){\textcolor{black}{$p_T=0.75$}}
    \end{overpic}
    \caption{Sparse input with 20K points up-sampled to 120K points.}
    \label{fig:plane_sparse}
\end{figure}

==> figures/004_experiments/sparse/sparse.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{figures/004_experiments/sparse/sparse.jpg} 
    \caption{Sparse input with 10K points up-sampled to 175K points.}
    \label{fig:sparse1}
\end{figure}

==> figures/004_experiments/sparse/spot.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{figures/004_experiments/sparse/spot.jpg} 
    \caption{50K points as input up-sampled to 600K points.}
    \label{fig:spot}
\end{figure}
